QuITO: Numerical software for constrained nonlinear optimal control problems -- extended version

We introduce the MATLAB-based software QuITO (Quasi-Interpolation based Trajectory Optimization) to numerically solve a wide class of constrained nonlinear optimal control problems (OCP). The solver is based on the QuITO (the same abbreviation) algorithm, which is a direct multiple shooting (DMS) technique that leverages a particular type of quasi-interpolation scheme for control trajectory parameterization. The software is equipped with several options for numerical integration, and optimization solvers along with a Graphical User Interface (GUI) to make the process of designing and solving the OCPs smooth and seamless for users with minimum coding experience. We demonstrate with two benchmark numerical examples the procedure to generate constrained state and control trajectories using QuITO.

==> concl.tex <==
%% =============================================================================
\section{Concluding remarks}
%% =============================================================================

We introduced QuIFS, an one-shot approximate feedback synthesis algorithm for nonlinear robust MPC problems which theoretically provide guarantees for uniform error estimates between the optimal and the approximate feedback policies.
% Our algorithm is a \emph{one-shot} synthesis mechanism --- given an error margin \(\eps>0\) one can pick three parameters namely the stepsize \(h>0\), the shape parameter \(\Dd>0\) and a number \(R_0>0\) related with the error between the actual and the truncated approximation engines, such that the optimal and the approximated feedbacks (in the sense of equation \eqref{eq:approx_policy} in \S\eqref{sec:extension_algo_step_three}) are \emph{uniformly} \(\eps\)-close. 
It was also shown that under the approximate policy \(\mutrunc(\cdot)\) the closed loop process related to the recursion \eqref{eq:system} is ISS-like stable (in the sense of Definition \eqref{appen_b_Regional_Practical_ISS}) and recursively feasible. One of the future direction of this work involves developing approximate robust MPC solvers leveraging very novel \cite{ref:DasAraCheCha-22}, \cite{ref:PP:DC:22} results on computable near-optimal solutions of convex semi-infinite problems. Natural extensions to the case of stochastic MPC are being developed and will be reported separately. 


